Embedded out-of-distribution detection on an autonomous robot platform

Machine learning (ML) is actively finding its way into modern cyber-physical systems (CPS), many of which are safety-critical real-time systems. It is well known that ML outputs are not reliable when testing data are novel with regards to model training and validation data, i.e., out-of-distribution (OOD) test data. We implement an unsupervised deep neural network-based OOD detector on a real-time embedded autonomous Duckiebot and evaluate detection performance. Our OOD detector produces a success rate of 87.5% for emergency stopping a Duckiebot on a braking test bed we designed. We also provide case analysis on computing resource challenges specific to the Robot Operating System (ROS) middleware on the Duckiebot.

==> Backup.tex <==
In recent years,  machine learning (ML) models have been used for accomplishing different tasks in cyberphysical systems (CPS) such as obgect detection, image segmentation and etc. However it is shown that the reliability of predictions provided by ML models is closely related to the training data \cite{gu2019towards}. As a result, ML models with low  error during training can have high  error during testing for unseen samples. Out of distribution detection (OOD) tries to adress this problem by indentifying test samples which have not been seen during training (OOD samples). Pervious approaches uses different models for identifying OOD samples. One of the common architectures which is used for identifying OOD samples is variational autoencoder (VAE) \cite{kingma2013auto} and its variants ($\beta $-VAE \cite{ramakrishna2020efficient}, conditional VAE \cite{vernekar2019out} and etc). VAE is formed by two connected neural netwrok named encoder and decoder. The encoder maps the input data to  encoded representation in  latent layer and the decoder reconstruct the image by sampling encodeed representation from hidden layer. The hidden layer usually has lower dimension than input layer and follows specific predifined distribution. The loss function of VAE consists of reconstruction loss and regularization term. Reconstruction loss makes sure the latent representation is meaningful and  contains the critical information required for reconstruction of image. The regulariztion term  prevents overfitting of the model \cite{kingma2013auto}. 
There two main types of appraoches which uses VAE as OOD detector, the approaches which use output space of VAE for OOD detection and approaches which use laten space of VAE for OOD detection and approaches which uses output space of VAE as OOD detector. Approaches which use output space of OOD use reconstruction loss or variant of that for OOD detection. In  \cite{amini2018variational}, the VAE is used for as OOD detector and it triggers the steering command based on road curvature. This appraoch uses pixelwise error between generated and orginal image as OOD score. The loss function of VAE in this setting consists of reconstruction loss, regularization term and  supervised latent loss. Supervised latent losss calculates the diffefrence betwen  true and predicted steering command which is encoded in specific latent varaible. In \cite{cai2020real}, the two phased approach which usues VAE as OOD detector is proposed. In both  offfline (training) and online (testing) phases the concept named inductive conformal prediction (ICP) \cite{} is used. For applying ICP framework,  the non-conformity score (the amount of surprise for given sample should be calculated). The non-conformity score is calculated as distance between original and reconstructed image.  In offline phase, first, the sample will be divided into training and calibration sets. Then the non-conformity score for calibration dataset is calculated. Then in online phase the non-conformity score for test sample is calculated. Afterthat, the p-value \cite{} for test sample is defined as ratio of validation data sets with non-conformity score more than predifined dataset. 
For using ICP framework one has to define non-conformity score. The non-conformity score calculates the amount of surprise for given test sample and in this paper  the  distance between reconstructed and original images is considered as nonconformity score.  

Our  approach  deploys the simplified version of framework \cite{}. In this approach first the $\beta$-VAE is trained and then latent space of $\beta$-VAE is used for OOD detection. For identifying the most informative latent units (latent units which capture important aspects of image), first, we feed a scene consisting of sequence of images to encoder of trained  $beta$-VAEand.  Next we extract two subsequent pair of images in the scene. After that for each dimension of latent space  we calculate the KL-divergence between learned distribution and prior distribution (Gaussian distribution). After that the KL-divergence for subsequent frames will be subracted from each other. 




In recent years,  machine learning (ML) models have been used for accomplishing different tasks in cyber-physical systems (CPS) such as object detection, image segmentation, etc. However, it is shown that the reliability of predictions provided by ML models is closely related to the quality of data \cite{gu2019towards}. As a result, ML models with a low error during training can have a high error during testing for unseen samples. Reliability of results for safe CPS is vital. In safe CPS systems such as autonomous cars  any mistake in provided result can lead to incompensable results such as individual death \cite{kohli2019enabling}. Out of distribution detection (OOD) tries to address this problem by identifying test samples that does not drawn from the  same distribution as training dataset (OOD samples) \cite{bulusu2020anomalous}. Previous approaches use different models for identifying OOD samples. One of the common architectures which is used for identifying OOD samples is variational autoencoder (VAE) \cite{kingma2013auto} and its variants ($\beta $-VAE \cite{ramakrishna2020efficient}, conditional VAE \cite{vernekar2019out} and etc). VAE is formed by two connected neural networks named encoder and decoder. The encoder maps the input data to encoded representation in the latent layer, and the decoder reconstructs the image by sampling encoded representation from the hidden layer. The hidden layer usually has lower dimension than the input layer and follows the specific predefined distribution. The loss function of VAE consists of reconstruction loss and a regularization term. Reconstruction loss makes sure the latent representation is meaningful and contains the critical information required to reconstruct the image. The regularization term prevents overfitting of the model \cite{kingma2013auto}. 
There two main types of approaches, which use VAE as an OOD detector, the approaches which use output space of VAE for OOD detection \cite{cai2020real,an2015variational,vasilev2020q,amini2018variational} and approaches which use latent space of VAE for OOD detection \cite{vasilev2020q,zhang2020out,ramakrishna2020efficient}. Approaches apply OOD detection on output space,  use reconstruction loss (for example, the pixel-wise difference between original and reconstructed image) or a variant of it for OOD detection. Such approaches calculate reconstruction loss based on likelihood., as mentioned in \cite{nalisnick2018deep} can produce higher likelihood (lower reconstruction loss for OOD data). In contrast, approaches that use latent space for detecting OOD samples show more reliable results. In this approach, the regularization term (usually calculated as KL-divergence \cite{cardoso1997infomax} between the prior distribution of latent space and learned distribution of latent space is used).
Our  approach  deploys the simplified version of framework \cite{ramakrishna2020efficient}. In this approach first the $\beta$-VAE is trained and then latent space of $\beta$-VAE is used for OOD detection. The most informative latent variables (OOD detectors) are identified based on their KL-divergence average over pair of images in a scene through all scenes of training set. The latent variables with the highest KL-divergence average are selected OOD detectors.

Although all these approaches provide a significant result, they only use simulators such as CARLA \cite{dosovitskiy2017carla} simulator \cite{ramakrishna2020efficient,cai2020real} or real-car test-bed \cite{amini2018variational} (this approach is based on reconstruction loss, and therefore it does not provide reliable results). As a result, none of them were tested in a real-time embedded test-bed with limited resources such as duckie-bot \cite{7989179}. Therefore in this work, we tried to deploy the $\beta$-VAE detector, which uses the latent space of VAE as an OOD detector to verify the practical aspects of such an approach. 











%%%%%%%%%%%%%%%%%%%%%%%%%%%5


In out of distribution detection (OOD) proablem, the goal is to identify  test samples  that does not drawn from the  same distribution as training dataset (OOD samples)  \cite{bulusu2020anomalous}. Previous approaches use different models for identifying OOD samples.
 The models used for OOD detection can be divided into discriminative and generative models. Generative models can learn data distribution directly and they have built-in dimension reduction mechanism which makes them scalable. In contrast to generative models, discriminative models, usually have higher performance and are interpretabale. In \cite{ruff2018deep}, the deep architecture for SVDD model is proposeed which mapped input space to hyper-sphere representationa and the distance from center of hyper-sphere is used for detecting OOD samples. However discriminative models even in their deep forms still are more resource intensive than generative models and they can lose their interpretability in deep form. As result using generative models for OOD detection is more common.
 The two main categories of models which is used as OOD detector are generative adversarial network (GAN) \cite{goodfellow2014generative}, variational autoencoder models (VAE) \cite{kingma2013auto}. The GAN model consits of a generator and discriminator networks. The generator tries to learn data distribution implicitly by synthesysing samples close to real samples and the discriminator tries to discern between real samples and generated samples. Training the GAN can be seen as game between generator and discriminator. The generator and discriminator will be optimized when the reach their equiblirum point. GAN based OOD detectors usually  generate synthatic OOD samples close to training samples at training stage to acheive more accurate boundry for discerning OOD and in-distribution samples. Then they use the obtained boundary  at a test time for identifyoing OOD samples\cite{kliger2018novelty}. GAN-based appraoches learn data distribution implicitly \cite{goodfellow2016nips}. In contrast VAE  \cite{kingma2013auto} and its variants ($\beta $-VAE \cite{ramakrishna2020efficient}, conditional VAE \cite{vernekar2019out} and etc) learn the data distribution explicitly which make them suitable for OOD detection task. VAE is formed by two connected neural networks named encoder and decoder. The encoder maps the input data to encoded representation in the latent layer, and the decoder reconstructs the image by sampling encoded representation from the hidden layer. The hidden layer usually has lower dimension than the input layer and follows the specific predefined distribution. The loss function of VAE consists of reconstruction loss and a regularization term. Reconstruction loss makes sure the latent representation is meaningful and contains the critical information required to reconstruct the image. The regularization term prevents overfitting of the model \cite{kingma2013auto}. 
There two main types of approaches, which use VAE as an OOD detector, the approaches which use output space of VAE for OOD detection \cite{cai2020real,an2015variational,vasilev2020q,amini2018variational} and approaches which use latent space of VAE for OOD detection \cite{vasilev2020q,zhang2020out,ramakrishna2020efficient}. Approaches apply OOD detection on output space,  use reconstruction loss (for example, the pixel-wise difference between original and reconstructed image) or a variant of it for OOD detection. Such approaches calculate reconstruction loss based on likelihood., as mentioned in \cite{nalisnick2018deep} can produce higher likelihood (lower reconstruction loss for OOD data). In contrast, approaches that use latent space for detecting OOD samples show more reliable results. In this approach, the regularization term (usually calculated as KL-divergence \cite{cardoso1997infomax} between the prior distribution of latent space and learned distribution of latent space is used).
Our  approach  deploys the simplified version of framework \cite{ramakrishna2020efficient}. In this approach first the $\beta$-VAE is trained and then latent space of $\beta$-VAE is used for OOD detection. The most informative latent variables (OOD detectors) are identified based on their KL-divergence average over pair of images in a scene through all scenes of training set. The latent variables with the highest KL-divergence average are selected OOD detectors.

Although all these approaches provide a significant result, they only use simulators such as CARLA \cite{dosovitskiy2017carla} simulator \cite{ramakrishna2020efficient,cai2020real} or real-car test-bed \cite{amini2018variational} (this approach is based on reconstruction loss, and therefore it does not provide reliable results). As a result, none of them were tested in a real-time embedded test-bed with limited resources such as duckie-bot \cite{7989179}. Therefore in this work, we tried to deploy the $\beta$-VAE detector, which uses the latent space of VAE as an OOD detector to verify the practical aspects of such an approach. 

==> Duckiebot for OOD (1)/Backup.tex <==
In recent years,  machine learning (ML) models have been used for accomplishing different tasks in cyberphysical systems (CPS) such as obgect detection, image segmentation and etc. However it is shown that the reliability of predictions provided by ML models is closely related to the training data \cite{gu2019towards}. As a result, ML models with low  error during training can have high  error during testing for unseen samples. Out of distribution detection (OOD) tries to adress this problem by indentifying test samples which have not been seen during training (OOD samples). Pervious approaches uses different models for identifying OOD samples. One of the common architectures which is used for identifying OOD samples is variational autoencoder (VAE) \cite{kingma2013auto} and its variants ($\beta $-VAE \cite{ramakrishna2020efficient}, conditional VAE \cite{vernekar2019out} and etc). VAE is formed by two connected neural netwrok named encoder and decoder. The encoder maps the input data to  encoded representation in  latent layer and the decoder reconstruct the image by sampling encodeed representation from hidden layer. The hidden layer usually has lower dimension than input layer and follows specific predifined distribution. The loss function of VAE consists of reconstruction loss and regularization term. Reconstruction loss makes sure the latent representation is meaningful and  contains the critical information required for reconstruction of image. The regulariztion term  prevents overfitting of the model \cite{kingma2013auto}. 
There two main types of appraoches which uses VAE as OOD detector, the approaches which use output space of VAE for OOD detection and approaches which use laten space of VAE for OOD detection and approaches which uses output space of VAE as OOD detector. Approaches which use output space of OOD use reconstruction loss or variant of that for OOD detection. In  \cite{amini2018variational}, the VAE is used for as OOD detector and it triggers the steering command based on road curvature. This appraoch uses pixelwise error between generated and orginal image as OOD score. The loss function of VAE in this setting consists of reconstruction loss, regularization term and  supervised latent loss. Supervised latent losss calculates the diffefrence betwen  true and predicted steering command which is encoded in specific latent varaible. In \cite{cai2020real}, the two phased approach which usues VAE as OOD detector is proposed. In both  offfline (training) and online (testing) phases the concept named inductive conformal prediction (ICP) \cite{} is used. For applying ICP framework,  the non-conformity score (the amount of surprise for given sample should be calculated). The non-conformity score is calculated as distance between original and reconstructed image.  In offline phase, first, the sample will be divided into training and calibration sets. Then the non-conformity score for calibration dataset is calculated. Then in online phase the non-conformity score for test sample is calculated. Afterthat, the p-value \cite{} for test sample is defined as ratio of validation data sets with non-conformity score more than predifined dataset. 
For using ICP framework one has to define non-conformity score. The non-conformity score calculates the amount of surprise for given test sample and in this paper  the  distance between reconstructed and original images is considered as nonconformity score.  

Our  approach  deploys the simplified version of framework \cite{}. In this approach first the $\beta$-VAE is trained and then latent space of $\beta$-VAE is used for OOD detection. For identifying the most informative latent units (latent units which capture important aspects of image), first, we feed a scene consisting of sequence of images to encoder of trained  $beta$-VAEand.  Next we extract two subsequent pair of images in the scene. After that for each dimension of latent space  we calculate the KL-divergence between learned distribution and prior distribution (Gaussian distribution). After that the KL-divergence for subsequent frames will be subracted from each other. 




In recent years,  machine learning (ML) models have been used for accomplishing different tasks in cyber-physical systems (CPS) such as object detection, image segmentation, etc. However, it is shown that the reliability of predictions provided by ML models is closely related to the quality of data \cite{gu2019towards}. As a result, ML models with a low error during training can have a high error during testing for unseen samples. Reliability of results for safe CPS is vital. In safe CPS systems such as autonomous cars  any mistake in provided result can lead to incompensable results such as individual death \cite{kohli2019enabling}. Out of distribution detection (OOD) tries to address this problem by identifying test samples that does not drawn from the  same distribution as training dataset (OOD samples) \cite{bulusu2020anomalous}. Previous approaches use different models for identifying OOD samples. One of the common architectures which is used for identifying OOD samples is variational autoencoder (VAE) \cite{kingma2013auto} and its variants ($\beta $-VAE \cite{ramakrishna2020efficient}, conditional VAE \cite{vernekar2019out} and etc). VAE is formed by two connected neural networks named encoder and decoder. The encoder maps the input data to encoded representation in the latent layer, and the decoder reconstructs the image by sampling encoded representation from the hidden layer. The hidden layer usually has lower dimension than the input layer and follows the specific predefined distribution. The loss function of VAE consists of reconstruction loss and a regularization term. Reconstruction loss makes sure the latent representation is meaningful and contains the critical information required to reconstruct the image. The regularization term prevents overfitting of the model \cite{kingma2013auto}. 
There two main types of approaches, which use VAE as an OOD detector, the approaches which use output space of VAE for OOD detection \cite{cai2020real,an2015variational,vasilev2020q,amini2018variational} and approaches which use latent space of VAE for OOD detection \cite{vasilev2020q,zhang2020out,ramakrishna2020efficient}. Approaches apply OOD detection on output space,  use reconstruction loss (for example, the pixel-wise difference between original and reconstructed image) or a variant of it for OOD detection. Such approaches calculate reconstruction loss based on likelihood., as mentioned in \cite{nalisnick2018deep} can produce higher likelihood (lower reconstruction loss for OOD data). In contrast, approaches that use latent space for detecting OOD samples show more reliable results. In this approach, the regularization term (usually calculated as KL-divergence \cite{cardoso1997infomax} between the prior distribution of latent space and learned distribution of latent space is used).
Our  approach  deploys the simplified version of framework \cite{ramakrishna2020efficient}. In this approach first the $\beta$-VAE is trained and then latent space of $\beta$-VAE is used for OOD detection. The most informative latent variables (OOD detectors) are identified based on their KL-divergence average over pair of images in a scene through all scenes of training set. The latent variables with the highest KL-divergence average are selected OOD detectors.

Although all these approaches provide a significant result, they only use simulators such as CARLA \cite{dosovitskiy2017carla} simulator \cite{ramakrishna2020efficient,cai2020real} or real-car test-bed \cite{amini2018variational} (this approach is based on reconstruction loss, and therefore it does not provide reliable results). As a result, none of them were tested in a real-time embedded test-bed with limited resources such as duckie-bot \cite{7989179}. Therefore in this work, we tried to deploy the $\beta$-VAE detector, which uses the latent space of VAE as an OOD detector to verify the practical aspects of such an approach. 











%%%%%%%%%%%%%%%%%%%%%%%%%%%5


In out of distribution detection (OOD) proablem, the goal is to identify  test samples  that does not drawn from the  same distribution as training dataset (OOD samples)  \cite{bulusu2020anomalous}. Previous approaches use different models for identifying OOD samples.
 The models used for OOD detection can be divided into discriminative and generative models. Generative models can learn data distribution directly and they have built-in dimension reduction mechanism which makes them scalable. In contrast to generative models, discriminative models, usually have higher performance and are interpretabale. In \cite{ruff2018deep}, the deep architecture for SVDD model is proposeed which mapped input space to hyper-sphere representationa and the distance from center of hyper-sphere is used for detecting OOD samples. However discriminative models even in their deep forms still are more resource intensive than generative models and they can lose their interpretability in deep form. As result using generative models for OOD detection is more common.
 The two main categories of models which is used as OOD detector are generative adversarial network (GAN) \cite{goodfellow2014generative}, variational autoencoder models (VAE) \cite{kingma2013auto}. The GAN model consits of a generator and discriminator networks. The generator tries to learn data distribution implicitly by synthesysing samples close to real samples and the discriminator tries to discern between real samples and generated samples. Training the GAN can be seen as game between generator and discriminator. The generator and discriminator will be optimized when the reach their equiblirum point. GAN based OOD detectors usually  generate synthatic OOD samples close to training samples at training stage to acheive more accurate boundry for discerning OOD and in-distribution samples. Then they use the obtained boundary  at a test time for identifyoing OOD samples\cite{kliger2018novelty}. GAN-based appraoches learn data distribution implicitly \cite{goodfellow2016nips}. In contrast VAE  \cite{kingma2013auto} and its variants ($\beta $-VAE \cite{ramakrishna2020efficient}, conditional VAE \cite{vernekar2019out} and etc) learn the data distribution explicitly which make them suitable for OOD detection task. VAE is formed by two connected neural networks named encoder and decoder. The encoder maps the input data to encoded representation in the latent layer, and the decoder reconstructs the image by sampling encoded representation from the hidden layer. The hidden layer usually has lower dimension than the input layer and follows the specific predefined distribution. The loss function of VAE consists of reconstruction loss and a regularization term. Reconstruction loss makes sure the latent representation is meaningful and contains the critical information required to reconstruct the image. The regularization term prevents overfitting of the model \cite{kingma2013auto}. 
There two main types of approaches, which use VAE as an OOD detector, the approaches which use output space of VAE for OOD detection \cite{cai2020real,an2015variational,vasilev2020q,amini2018variational} and approaches which use latent space of VAE for OOD detection \cite{vasilev2020q,zhang2020out,ramakrishna2020efficient}. Approaches apply OOD detection on output space,  use reconstruction loss (for example, the pixel-wise difference between original and reconstructed image) or a variant of it for OOD detection. Such approaches calculate reconstruction loss based on likelihood., as mentioned in \cite{nalisnick2018deep} can produce higher likelihood (lower reconstruction loss for OOD data). In contrast, approaches that use latent space for detecting OOD samples show more reliable results. In this approach, the regularization term (usually calculated as KL-divergence \cite{cardoso1997infomax} between the prior distribution of latent space and learned distribution of latent space is used).
Our  approach  deploys the simplified version of framework \cite{ramakrishna2020efficient}. In this approach first the $\beta$-VAE is trained and then latent space of $\beta$-VAE is used for OOD detection. The most informative latent variables (OOD detectors) are identified based on their KL-divergence average over pair of images in a scene through all scenes of training set. The latent variables with the highest KL-divergence average are selected OOD detectors.

Although all these approaches provide a significant result, they only use simulators such as CARLA \cite{dosovitskiy2017carla} simulator \cite{ramakrishna2020efficient,cai2020real} or real-car test-bed \cite{amini2018variational} (this approach is based on reconstruction loss, and therefore it does not provide reliable results). As a result, none of them were tested in a real-time embedded test-bed with limited resources such as duckie-bot \cite{7989179}. Therefore in this work, we tried to deploy the $\beta$-VAE detector, which uses the latent space of VAE as an OOD detector to verify the practical aspects of such an approach. 

==> Duckiebot for OOD (1)/Duckiebotselection.tex <==

We select Duckiebot as an embedded platform for deploying the OOD detection algorithm. One of the main reasons behind this selection is that Duckiebot uses a robotic operating system (ROS). By considering autonomous car development frameworks such as Autoware \cite{kato2015open} which are based on ROS, our approach can be adapt and deployed on real autonomous cars. Also,  the challenges using ROS impose in the deployment phase in Duckiebot controlled settings can be used as a guideline for deploying an approach in any other ROS-based autonomous vehicle platform.



==> Duckiebot for OOD (1)/Related-Backup.tex <==
\section{Out-of-Distribution Detection}

The goal of the out-of-distribution detection (OOD) problem is to identify test samples that are not drawn from the same distribution as the training dataset (OOD samples)\cite{bulusu2020anomalous}. Previous approaches use different models for identifying OOD samples.
The models used for OOD detection can be divided into discriminative and generative models. Generative models can learn the data distribution directly, and they have a built-in dimension reduction mechanism that makes them scalable. In contrast to generative models, discriminative models usually have higher performance. In \cite{ruff2018deep}, the deep architecture for the SVDD model is proposed, which maps input space to a  hyper-sphere representation, and the distance from the center of the hyper-sphere is used for detecting OOD samples. However, discriminative models in their deep forms are more resource-intensive than generative models. As a result, using generative models for OOD detection is more common. The two main categories of models which are used as OOD detectors are generative adversarial network (GAN) \cite{goodfellow2014generative} and variational autoencoder models (VAE) \cite{kingma2013auto}. 

The GAN  consists of generator and discriminator networks. The generator tries to learn data distribution implicitly by synthesizing samples similar to real samples, and the discriminator tries to discern between real samples and generated samples. GAN-based OOD detectors usually generate synthetic OOD samples close to training samples at the training stage to achieve a more accurate boundary for discerning OOD and in-distribution samples. Then they use the obtained boundary at test time for identifying OOD samples\cite{kliger2018novelty}.

In contrast to GAN-based approaches which learn data distribution implicitly \cite{goodfellow2016nips}, approaches using VAE\cite{kingma2013auto} and its variants ($\beta $-VAE \cite{ramakrishna2020efficient}, conditional VAE \cite{vernekar2019out}, etc) learn the data distribution explicitly which make them more suitable for OOD detection tasks. VAE is formed by two connected neural networks named encoder and decoder. The encoder maps the input data to an encoded representation in the latent layer, and the decoder reconstructs the image by sampling an encoded representation from the hidden layer. The hidden layer usually has a lower dimension than the input layer and follows the specific predefined distribution. The loss function of VAE consists of reconstruction loss and a regularization term. Reconstruction loss ensures the latent representation is meaningful and contains the critical information required to reconstruct the image. The regularization term prevents overfitting of the model\cite{kingma2013auto}. 
There are two main types of approaches, which use VAE as an OOD detector, the approaches which use output space of VAE for OOD detection \cite{cai2020real,an2015variational,vasilev2020q,amini2018variational} and approaches which use latent space of VAE for OOD detection \cite{vasilev2020q,zhang2020out,ramakrishna2020efficient}. Approaches that apply OOD detection on output space,  use reconstruction loss (for example, the pixel-wise difference between original and reconstructed image) or a variation of it for OOD detection.  As mentioned in \cite{nalisnick2018deep}, approaches that calculate reconstruction loss based on likelihood can produce higher likelihood (lower reconstruction loss) for OOD data. In contrast, approaches that use latent space for detecting OOD samples show more reliable results. In latent space-based approaches, the regularization term (usually calculated as KL-divergence \cite{cardoso1997infomax} between the prior distribution of latent space and the learned distribution of latent space) is used for OOD detection.


Although all these approaches provide significant outcomes, they have only been deployed on simulators such as CARLA \cite{dosovitskiy2017carla} or real-car test-beds.  For example in \cite{ramakrishna2020efficient,cai2020real} CARLA simulator was used and in \cite{amini2018variational} a real car was used, although this approach is based on reconstruction loss, and therefore it does not provide reliable results. As a result, none of them were tested in a real-time embedded test-bed with limited resources. Therefore in this work, we deploy the OOD detector introduced in  \cite{ramakrishna2020efficient} on duckiebot \cite{7989179} to show the practicality of the current approach in the embedded setting. In this approach, first, the $\beta$-VAE is trained, and then the latent space of $\beta$-VAE is used to select the OOD detector. The OOD detectors are identified based on their KL-divergence average over pair of images in a scene through all scenes of the training set. The latent variables with the highest KL-divergence average are selected OOD detectors. The OOD sample can then be identified by monitoring this detector for a given test sample. 


==> Duckiebotselection.tex <==

We select Duckiebot as an embedded platform for deploying the OOD detection algorithm. One of the main reasons behind this selection is that Duckiebot uses a robotic operating system (ROS). By considering autonomous car development frameworks such as Autoware \cite{kato2015open} which are based on ROS, our approach can be adapt and deployed on real autonomous cars. Also,  the challenges using ROS impose in the deployment phase in Duckiebot controlled settings can be used as a guideline for deploying an approach in any other ROS-based autonomous vehicle platform.



==> Related-Backup.tex <==
\section{Out-of-Distribution Detection}

The goal of the out-of-distribution detection (OOD) problem is to identify test samples that are not drawn from the same distribution as the training dataset (OOD samples)\cite{bulusu2020anomalous}. Previous approaches use different models for identifying OOD samples.
The models used for OOD detection can be divided into discriminative and generative models. Generative models can learn the data distribution directly, and they have a built-in dimension reduction mechanism that makes them scalable. In contrast to generative models, discriminative models usually have higher performance. In \cite{ruff2018deep}, the deep architecture for the SVDD model is proposed, which maps input space to a  hyper-sphere representation, and the distance from the center of the hyper-sphere is used for detecting OOD samples. However, discriminative models in their deep forms are more resource-intensive than generative models. As a result, using generative models for OOD detection is more common. The two main categories of models which are used as OOD detectors are generative adversarial network (GAN) \cite{goodfellow2014generative} and variational autoencoder models (VAE) \cite{kingma2013auto}. 

The GAN  consists of generator and discriminator networks. The generator tries to learn data distribution implicitly by synthesizing samples similar to real samples, and the discriminator tries to discern between real samples and generated samples. GAN-based OOD detectors usually generate synthetic OOD samples close to training samples at the training stage to achieve a more accurate boundary for discerning OOD and in-distribution samples. Then they use the obtained boundary at test time for identifying OOD samples\cite{kliger2018novelty}.

In contrast to GAN-based approaches which learn data distribution implicitly \cite{goodfellow2016nips}, approaches using VAE\cite{kingma2013auto} and its variants ($\beta $-VAE \cite{ramakrishna2020efficient}, conditional VAE \cite{vernekar2019out}, etc) learn the data distribution explicitly which make them more suitable for OOD detection tasks. VAE is formed by two connected neural networks named encoder and decoder. The encoder maps the input data to an encoded representation in the latent layer, and the decoder reconstructs the image by sampling an encoded representation from the hidden layer. The hidden layer usually has a lower dimension than the input layer and follows the specific predefined distribution. The loss function of VAE consists of reconstruction loss and a regularization term. Reconstruction loss ensures the latent representation is meaningful and contains the critical information required to reconstruct the image. The regularization term prevents overfitting of the model\cite{kingma2013auto}. 
There are two main types of approaches, which use VAE as an OOD detector, the approaches which use output space of VAE for OOD detection \cite{cai2020real,an2015variational,vasilev2020q,amini2018variational} and approaches which use latent space of VAE for OOD detection \cite{vasilev2020q,zhang2020out,ramakrishna2020efficient}. Approaches that apply OOD detection on output space,  use reconstruction loss (for example, the pixel-wise difference between original and reconstructed image) or a variation of it for OOD detection.  As mentioned in \cite{nalisnick2018deep}, approaches that calculate reconstruction loss based on likelihood can produce higher likelihood (lower reconstruction loss) for OOD data. In contrast, approaches that use latent space for detecting OOD samples show more reliable results. In latent space-based approaches, the regularization term (usually calculated as KL-divergence \cite{cardoso1997infomax} between the prior distribution of latent space and the learned distribution of latent space) is used for OOD detection.


Although all these approaches provide significant outcomes, they have only been deployed on simulators such as CARLA \cite{dosovitskiy2017carla} or real-car test-beds.  For example in \cite{ramakrishna2020efficient,cai2020real} CARLA simulator was used and in \cite{amini2018variational} a real car was used, although this approach is based on reconstruction loss, and therefore it does not provide reliable results. As a result, none of them were tested in a real-time embedded test-bed with limited resources. Therefore in this work, we deploy the OOD detector introduced in  \cite{ramakrishna2020efficient} on duckiebot \cite{7989179} to show the practicality of the current approach in the embedded setting. In this approach, first, the $\beta$-VAE is trained, and then the latent space of $\beta$-VAE is used to select the OOD detector. The OOD detectors are identified based on their KL-divergence average over pair of images in a scene through all scenes of the training set. The latent variables with the highest KL-divergence average are selected OOD detectors. The OOD sample can then be identified by monitoring this detector for a given test sample. 

